Disentangling Video with Independent Prediction

We propose an unsupervised variational model for disentangling video into independent factors, i.e. each factor's future can be predicted from its past without considering the others. We show that our approach often learns factors which are interpretable as objects in a scene.

==> makefile <==
all: html pdf

pdf-figures:
	@./pdf-figures.fish
	@echo "SVG figures compiled to PDF."

pdf:
	@pandoc main.md \
		--number-sections \
		--filter pandoc-crossref \
		--filter pandoc-citeproc \
		--template pandoc_template.tex \
		-o output/rendered.pdf 2>&1
	@echo "PDF rendered successfully."

tex:
	@pandoc main.md \
		--number-sections \
		--filter pandoc-crossref \
		--filter pandoc-citeproc \
		--template pandoc_template.tex \
		-o output/rendered.tex

html:
	@pandoc main.md \
		--number-sections \
		--filter pandoc-crossref \
		--filter pandoc-citeproc \
		-s \
		--to html5 \
		-o output/rendered.html --mathjax

pdf-and-notify:
	@make pdf \
		| xargs -I XXX sh -c "echo 'XXX' && osascript -e 'display notification \"XXX\" with title \"Document generation output\"';"

watch:
	@# reload -b -s output/rendered.html & make html & fswatch -o *.md */*.md | xargs -n1 make html
	-@make pdf
	@fswatch -o *.md */*.md \
		| xargs -n1 -I XXX make pdf-and-notify

watch-figures:
	@make pdf-figures
	@make pdf
	@fswatch -o figures/*.svg \
		| xargs -n1 -I XXX make pdf-figures \
		| xargs -I XXX make pdf-and-notify

install-deps:
	curl -sSL https://get.haskellstack.org/ | sh
	stack setup
	stack install pandoc pandoc-citeproc pandoc-crossref
	brew install fswatch


==> variational-factorized-model arxiv submission/makefile <==
all: html pdf

pdf-figures:
	@./pdf-figures.fish
	@echo "SVG figures compiled to PDF."

pdf:
	@pandoc main.md \
		--number-sections \
		--filter pandoc-crossref \
		--filter pandoc-citeproc \
		--template pandoc_template.tex \
		-o output/rendered.pdf 2>&1
	@echo "PDF rendered successfully."

tex:
	@pandoc main.md \
		--number-sections \
		--filter pandoc-crossref \
		--filter pandoc-citeproc \
		--template pandoc_template.tex \
		-o output/rendered.tex

html:
	@pandoc main.md \
		--number-sections \
		--filter pandoc-crossref \
		--filter pandoc-citeproc \
		-s \
		--to html5 \
		-o output/rendered.html --mathjax

pdf-and-notify:
	@make pdf \
		| xargs -I XXX sh -c "echo 'XXX' && osascript -e 'display notification \"XXX\" with title \"Document generation output\"';"

watch:
	@# reload -b -s output/rendered.html & make html & fswatch -o *.md */*.md | xargs -n1 make html
	-@make pdf
	@fswatch -o *.md */*.md \
		| xargs -n1 -I XXX make pdf-and-notify

watch-figures:
	@make pdf-figures
	@make pdf
	@fswatch -o figures/*.svg \
		| xargs -n1 -I XXX make pdf-figures \
		| xargs -I XXX make pdf-and-notify

install-deps:
	curl -sSL https://get.haskellstack.org/ | sh
	stack setup
	stack install pandoc pandoc-citeproc pandoc-crossref
	brew install fswatch

